LENS: Localization enhanced by NeRF synthesis

Neural Radiance Fields (NeRF) have recently demonstrated photo-realistic results for the task of novel view synthesis. In this paper, we propose to apply novel view synthesis to the robot relocalization problem: we demonstrate improvement of camera pose regression thanks to an additional synthetic dataset rendered by the NeRF class of algorithm. To avoid spawning novel views in irrelevant places we selected virtual camera locations from NeRF internal representation of the 3D geometry of the scene. We further improved localization accuracy of pose regressors using synthesized realistic and geometry consistent images as data augmentation during training. At the time of publication, our approach improved state of the art with a 60% lower error on Cambridge Landmarks and 7-scenes datasets. Hence, the resulting accuracy becomes comparable to structure-based methods, without any architecture modification or domain adaptation constraints. Since our method allows almost infinite generation of training data, we investigated limitations of camera pose regression depending on size and distribution of data used for training on public benchmarks. We concluded that pose regression accuracy is mostly bounded by relatively small and biased datasets rather than capacity of the pose regression model to solve the localization task.

==> sections/method_prev.tex <==
\section{Synthetic dataset rendering with LENS}
\label{sec:method}

We provide here a description of our method, which can be seen as an offline data augmentation pipeline. Our goal is to generate a large and uniformly distributed dataset of synthetic images, using a small set of images depicting the scene labeled with reference camera poses (usually provided by structure from motion methods such as COLMAP~\citep{colmap}). This dataset is then used to train a camera pose regressor, resulting in an improved accuracy without additional computation during localization inference. Our framework is described in figure~\ref{fig:method} and is detailed below.

\begin{figure}[h]
    \begin{center}
        \includegraphics[width=\linewidth]{figures/method2.png}
    \end{center}
    \caption{\textbf{LENS pipeline:} First, NeRF-W is trained with available real images. Then, the model is used to detect high density points in the scene. Poses from real images and high density are used to generate pose queries on which novel view synthesis is performed. Real and synthetic datasets are used to train a image pose regressor, which is used for real-time camera relocalization.}\label{fig:method}
\end{figure}

\subsection{Novel view synthesis with Nerf-W}

A neural radiance field performs novel view synthesis thanks to multilayer perceptrons (MLP) which learn to connect a 3D position $\bf{x} = (x,y,z)$ and a viewing direction $\bf{d}$ in a given scene to one density value $\sigma$ and one color $\bf{c}=(r,g,b)$. To render an image from a given position and camera orientation, inference is performed by sampling points along rays. The final RGB value of a pixel $\bf{C}$ is computed by approximating the volume rendering integral using $N$ samples $(t_{i})_{n}$ with predicted colors $(\bf{c}_{i})_{n}$ and densities $(\sigma_{i})_{n}$:
\begin{equation}
    C(r) = \sum_{i}^{n}{T_{i}(1-\exp{(-\sigma_{i}\delta_{i})})\bf{c}_{i}} 
    \quad\mathrm{where}\quad 
    T_{i} = \exp{(-\sum_{j=1}^{i-1}{\sigma_{j}\delta_{j}})}
    \quad\mathrm{and}\quad 
    \delta_{i} = t_{i+1} - t_{i}
\end{equation}
With this formulation, NeRF models are able to render a static scene captured under controlled settings but fail in real world dynamic scenes with variable illuminations and dynamic objects. NeRF in the Wild~\citep{nerfw} (NeRF-W), overcomes this limitation by modelling these temporal modifications with learned latent spaces that provide control on the appearance of each rendered view. 

We decide to use this method to generate our synthetic images: a NeRF-W model is trained on each scene thanks to a training dataset of real images. Then novel views are synthesised on each virtual camera location (see \ref{subsec:pose_query}), with appearance randomly interpolated from appearances embeddings of training set images.
As a result, rendered images depict a scene from chosen viewpoints where transient occluders observed in training images are removed. Appearance interpolation acts as a data augmentation technique that increases robustness of the localization model under varying illuminations. Some example of resulting appearances are shown in figure~\ref{fig:appearances}.

\subsection{Virtual camera locations from NeRF scene density volume}
\label{subsec:pose_query}

\input{tables/visualization}

One of the challenges we face is the choice of virtual camera locations where the images will be rendered. We emphasize that we are constructing a training dataset, and therefore a particular attention should be paid to the distribution of poses. We want this distribution to be uniform in the set of realistic camera viewpoints (\textit{i.e.} locations that can be visited by the robot). To do so, we compute a regular grid of points around real images poses, similar to~\citep{24-7}. However, some of these views are possibly occluded by objects and buildings or depict an area of the scene which is not represented in the real images. We observed that such camera locations are counter productive for localization accuracy so we use the NeRF's learned geometry structure of the scene and discard views occluded by these high density points.

Scene density volume is computed by forward passes on the first MLP of NeRF-W, that takes a 3d point $(x,y,z)$ as input and output a density $\sigma$, which can be interpreted as the density of matter at a given location. We query this MLP on a regular 3D grid and store results, that can be displayed as a density volume (see figure~\ref{fig:method}). To consider that a given location is unreachable in the scene, we set a threshold $t_\sigma$ and only take in account 3D points with an density higher than $t_\sigma$.
%For our algorithm, we store  with density higher than 20 (empirical threshold provided by \cite{nerfw_pytorch}) as a 3D point cloud.

Our virtual camera locations algorithm takes as input the poses of real images, the NeRF density volume and the desired number of virtual cameras $n$. D
%Depending on the application, one might want to sample points in 2D or 3D (a camera mounted on a vehicle always have same altitude at a given 2d location), our method works for both cases.
The first step is to chose camera locations, then an orientation is attached to each translation vector.

First, a regular grid is defined in a rectangle (2D case) or a rectangular parallelepiped (3D) where edges are set by extrema of training set poses for each dimension to which we add an extrapolation distance parameter $E_{max}$. Then, grid points that are too far from training set locations or too close from high density points are discarded. We implement this step with KDTrees for an efficient nearest neighbour search. If the number of valid points is lower than the number of queries, we iteratively increase the grid resolution and repeat the process.

Finally, we need to define a camera orientation $(qx,qy,qz,qw)$ attached to the camera center $(x,y,z)$ for each virtual camera. In order to avoid degenerate views, we copy the orientation of the nearest pose in training set and add a small random perturbations along the three 3D axis $(\zeta_x,\zeta_y, \zeta_z)$. This perturbation is implemented by multiplying the orientation with basic rotation matrices of each axis defined with a random angle $\zeta_d, d \in [x, y, z]$ drawn uniformly in $[-\frac{\zeta_d}{2},\frac{\zeta_d}{2}]$. 
%where $\theta$ is a parameter that we usually set to 15°.

As an output, we have a set of $n$ poses $[x,y,z,qx,qy,qz,qw]$ that are used as queries for novel view synthesis.

\subsection{Train a camera pose regressor with rendered images}

The final step of our pipeline is to train the localization algorithm with the synthetic dataset. Obviously, a domain gap exists between real and synthetic images : no dynamic objects, different textures, more blur and some artefacts are observable in the synthetic domain. As a result, training only with synthetic data leads to poor performances on real images. One simple solution to improve the robustness across domains is to use both real and synthetic images during training. Our method simply gathers both datasets together and mini-batchs are sampled randomly in this fused dataset. We tried to enforce a fixed percentage of real data in mini-batchs but did not observe improvements over random sampling.

We evaluated our method using CoordiNet~\cite{CoordiNet} as camera pose regressor. CoordiNet is a CNN that uses inductive biases in the network architecture that facilitate geometrical reasoning for the localization task, and also provides an uncertainty quantification for each pose that can be used as a covariance matrix. However, we suppose that using LENS as an additional training dataset improves the performance of any pose regression network.

After training, real-time localization is achieved by a single forward pass on the camera pose regressor, which is one of the main advantage of camera pose regression over other visual localizations methods.

\begin{figure}[h]
    \begin{center}
        \includegraphics[width=\linewidth]{figures/appearances.png}
    \end{center}
    \caption{Examples of images rendered from the same views with appearances sampled by random interpolation of appearance embeddings.}\label{fig:appearances}
\end{figure}

==> sections/prev_abstract.tex <==
Camera pose regression algorithms are an appealing solution for robot or vehicle localization systems. These neural networks can regress camera position and orientation in a known environment with a single image in an efficient way compared to other visual-based localization algorithms. However, accuracy of these learning-based methods is highly dependent on quantity and diversity of training data. We present a method that uses Neural Radiance Fields (NeRF) to generate synthetic images with novel views and appearance augmentations. These rendered images are gathered to create a training dataset which is distributed uniformly on possible camera view points. Thanks to the quality of novel view synthesis provided by NeRF, we show that algorithms trained with this synthetic data have a significantly better performance on real world images without any modification in the architecture or domain adaptation constraints. In addition with quantity, our data augmentation method increases diversity in the images because views are sampled on a regular grid across the possible poses, that we retrieve thanks to NeRF density estimation. Experiments made on indoor and outdoor scenes show that camera pose regression is currently limited because training datasets are too small and biased for a deep learning approach, and that novel view rendering is a way to mitigate this issue.

==> tables/Cambridge_SOTA.tex <==

\begin{table}[h]
\begin{tabular}{cl|l|l|l|l|l|}
\cline{3-7}
\multicolumn{1}{l}{\textbf{}} &
  \textbf{} &
  \multicolumn{1}{c|}{Kings} &
  \multicolumn{1}{c|}{Hospital} &
  \multicolumn{1}{c|}{Shop} &
  \multicolumn{1}{c|}{Church} &
  \multicolumn{1}{c|}{\textbf{Average}} \\ \hline
\multicolumn{1}{|c|}{\multirow{4}{*}{CPR}} & PoseNet \cite{geometric_loss_function}                 & 0.99/1.1  & 2.17/2.9 & 1.05/4.0 & 1.49/3.4 & 1.43/2.9 \\ \cline{2-2}
\multicolumn{1}{|c|}{}                     & TransPoseNet \cite{TransPoseNet}            & 0.60/2.43 & 1.45/3.1 & 0.55/3.5 & 1.09/5.0 & 0.91/3.5 \\ \cline{2-2}
\multicolumn{1}{|c|}{}                     & CoordiNet \cite{CoordiNet}               & 0.70/0.9  & 0.97/2.1 & 0.69/3.7 & 1.32/3.6 & 0.92/2.6 \\ \cline{2-2}
\multicolumn{1}{|c|}{}                     & \textbf{CoordiNet+LENS} &           &          & 0.27/1.6 &          &          \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{3D}}  & Active search \cite{activesearch}            & 0.42/0.6  & 0.44/1.0 & 0.12/0.4 & 0.19/0.5 & 0.29/0.6 \\ \cline{2-2}
\multicolumn{1}{|c|}{}                     & DSAC* \cite{dsac}                   & 0.18/0.3  & 0.21/0.4 & 0.05/0.3 & 0.15/0.6 & 0.15/0.4 \\ \hline
\end{tabular}
\caption{\label{tab:cambridge_results} Benefits of LENS on Cambridge Landmarks dataset.}
\end{table}


==> tables/SOTA_comparison.tex <==
\begin{table}[h]
%\begin{tabular}{l|llllll}
\small
\begin{tabular}{l|cccccc}
Dataset     & \multicolumn{4}{c|}{\hfil Camera pose regression}                       & \multicolumn{1}{l|}{3D}       & SCR      \\ \hline
Cambridge & \multicolumn{1}{p{1cm}}{PN \cite{geometric_loss_function}}  & \multicolumn{1}{p{1.7cm}}{TransPoseNet \cite{TransPoseNet}} & \multicolumn{1}{p{1cm}}{CoordiNet \cite{CoordiNet}} & \multicolumn{1}{p{1.5cm}|}{\textbf{CoordiNet + LENS}} & \multicolumn{1}{p{1.7cm}|}{Active Search \cite{activesearch}} &
\multicolumn{1}{p{1.5cm}}{DSAC* \cite{dsac}}  
\\ \hline
K College  & 0.99/1.1 & 0.60/2.4     & 0.70/0.9  & \multicolumn{1}{l|}{\bf{0.33/0.5}}         & \multicolumn{1}{l|}{0.42/0.6}      & 0.18/0.3 \\
O Hospital & 2.17/2.9  & 1.45/3.1  & 0.97/2.1  & \multicolumn{1}{l|}{\bf{0.44/0.9}}         & \multicolumn{1}{l|}{0.44/1.0} & 0.21/0.4 \\
S Facade    & 1.05/4.0 & 0.55/3.5     & 0.69/3.7  & \multicolumn{1}{l|}{\bf{0.27/1.6}}         & \multicolumn{1}{l|}{0.12/0.4}      & 0.05/0.3 \\
Church & 1.49/3.4 & 1.09/5.0     & 1.32/3.6  & \multicolumn{1}{l|}{\bf{0.53/1.6}}         & \multicolumn{1}{l|}{0.19/0.5}      & 0.15/0.6 \\ \hline
Average     & 1.43/2.9  & 0.91/3.5  & 0.92/2.6  & \multicolumn{1}{l|}{\bf{0.39/1.2}}         & \multicolumn{1}{l|}{0.29/0.6} & 0.15/0.4 \\ \hline
7scenes     &           &           &           &                               &                               &          \\ \hline
Chess       & 0.14/4.5  & 0.08/5.7  & 0.14/6.7  & \multicolumn{1}{l|}{\bf{0.03/1.3}} & \multicolumn{1}{l|}{0.04/2.0} & 0.02/1.1 \\
Fire        & 0.27/11.8 & 0.24/10.6 & 0.27/11.6 & \multicolumn{1}{l|}{\bf{0.10/3.7}} & \multicolumn{1}{l|}{0.03/1.5} & 0.02/1.2 \\
Heads       & 0.18/12.1 & 0.13/12.7 & 0.13/13.6 & \multicolumn{1}{l|}{\bf{0.07/5.8}} & \multicolumn{1}{l|}{0.02/1.5} & 0.01/1.8 \\
Office      & 0.20/5.8  & 0.17/6.3  & 0.21/8.6  & \multicolumn{1}{l|}{\bf{0.07/1.9}} & \multicolumn{1}{l|}{0.09/3.6} & 0.03/1.2 \\
Pumpkin     & 0.25/4.8  & 0.17/5.6  & 0.25/7.2  & \multicolumn{1}{l|}{\bf{0.08/2.2}} & \multicolumn{1}{l|}{0.08/3.1} & 0.04/1.4 \\
Kitchen     & 0.24/5.5  & 0.19/6.8  & 0.26/7.5  & \multicolumn{1}{l|}{\bf{0.09/2.2}} & \multicolumn{1}{l|}{0.07/3.4} & 0.03/1.7 \\
Stairs      & 0.37/10.6 & 0.30/7.0  & 0.28/12.9 & \multicolumn{1}{l|}{\bf{0.14/3.6}} & \multicolumn{1}{l|}{0.03/2.2} & 0.04/1.4 \\ \hline
Average     & 0.24/7.9  & 0.18/7.8  & 0.22/9.7  & \multicolumn{1}{l|}{\bf{0.08/3.0}} & \multicolumn{1}{l|}{0.05/2.5} & 0.03/1.4 \\ \hline
\end{tabular}
\caption{\label{tab:sota_results} \textbf{6DOF median localization errors of visual localization methods.}}
\end{table}

==> tables/visualization.tex <==
\begin{table}[t]
%\begin{tabular}{m{3cm} m{3cm} m{3cm} m{3cm} m{3cm} m{3cm}}
\small
\begin{tabular}{m{0.1cm} p{4cm} p{4cm} p{4cm}}
\begin{sideways} Shop \end{sideways} &
\begin{minipage}{4cm}
    \includegraphics[width=\linewidth]{figures/visualization_images/ShopFacade/volume.JPG}
\end{minipage} &
\begin{minipage}{4cm}
    \includegraphics[width=\linewidth]{figures/visualization_images/ShopFacade/poses.JPG}
\end{minipage} &
\begin{minipage}{4cm}
    \includegraphics[width=\linewidth]{figures/visualization_images/ShopFacade/sample1.jpg}
\end{minipage}
\\
\begin{sideways} Kings \end{sideways} &
\begin{minipage}{4cm}
    \includegraphics[width=\linewidth]{figures/visualization_images/KingsCollege/volume.JPG}
\end{minipage} &
\begin{minipage}{4cm}
    \includegraphics[width=\linewidth]{figures/visualization_images/KingsCollege/poses.JPG}
\end{minipage} &
\begin{minipage}{4cm}
    \includegraphics[width=\linewidth]{figures/visualization_images/KingsCollege/sample1.jpg}
\end{minipage}
\\
\begin{sideways} Hospital \end{sideways} &
\begin{minipage}{4cm}
    \includegraphics[width=\linewidth]{figures/visualization_images/OldHospital/volume.JPG}
\end{minipage} &
\begin{minipage}{4cm}
    \includegraphics[width=\linewidth]{figures/visualization_images/OldHospital/poses.JPG}
\end{minipage} &
\begin{minipage}{4cm}
    \includegraphics[width=\linewidth]{figures/visualization_images/OldHospital/sample1.jpg}
\end{minipage}
\\
\begin{sideways} Church \end{sideways} &
\begin{minipage}{3.7cm}
    \includegraphics[width=\linewidth]{figures/visualization_images/Church/volume.JPG}
\end{minipage} &
\begin{minipage}{4cm}
    \includegraphics[width=\linewidth]{figures/visualization_images/Church/poses.JPG}
\end{minipage} &
\begin{minipage}{4cm}
    \includegraphics[width=\linewidth]{figures/visualization_images/Church/sample1.jpg}
\end{minipage}
\end{tabular}
\captionof{figure}{Visualisation of density volumes, virtual camera queries (\textcolor{Green}{training poses}, \textcolor{blue}{test poses},\textcolor{red}{virtual cameras}) and example of rendered images on Cambridge Landmarks. }
\label{fig:viz}
\end{table}
